Learning Multimodal Latent Space with EBM Prior and MCMC Inference

Multimodal generative models are crucial for various applications. We propose an approach that combines an expressive energy-based model (EBM) prior with Markov Chain Monte Carlo (MCMC) inference in the latent space for multimodal generation. The EBM prior acts as an informative guide, while MCMC inference, specifically through short-run Langevin dynamics, brings the posterior distribution closer to its true form. This method not only provides an expressive prior to better capture the complexity of multimodality but also improves the learning of shared latent variables for more coherent generation across modalities. Our proposed method is supported by empirical experiments, underscoring the effectiveness of our EBM prior with MCMC inference in enhancing cross-modal and joint generative tasks in multimodal contexts.

==> sec/3_method_v1.tex <==
\section{Methodology}
In this work, we present a novel framework for effectively modeling multimodalities. In particular, we propose a joint training scheme with an EBM prior and MCMC inference, abbreviated as EBM-MCMC.

\subsection{Latent-space Multimodal}

\noindent \textbf{Latent-space Generative Model} In latent generative models, the complete data can be expressed as $p_{\theta}(x, z) = p_{\alpha}(z)p_{\beta}(x|z)$. Let $x \in \mathbb{R}^{D}$ represent the observed data, and $z \in \mathbb{R}^{d}$ represent the latent variables of $x$. The joint distribution of the data and latent variables ($x$, $z$) is learned through maximum likelihood estimation (MLE). 
% {
% \small
% \begin{equation}
%     \begin{aligned}
%     \label{eqn:complete_joint}
%         &p_{\theta}(x, z) = p_{\alpha}(z)p_{\beta}(x|z)
%     \end{aligned}
% \end{equation}}
\\
\noindent \textbf{Latent-space Multimodality Generative Model} In a multimodal context with a latent space, the joint distribution is factorized into a prior distribution and likelihood for each modality, as shown in Eqn. \ref{eqn:multimodal_complete_joint}, 
{
\small
\begin{equation}
\begin{aligned}
\label{eqn:multimodal_complete_joint}
&\prod_{i = 1}^{m} p_{\theta}(x^{(i)}, z) = p_{\alpha}(z)p_{\beta{(0)}}(x^{(0)}|z) \cdots p_{\beta{(i)}}(x^{(i)}|z)
\end{aligned}
\end{equation}
}
where $p_{\alpha}(z)$ represents the prior distribution and $p_{\beta{(i)}}(x^{(i)}|z)$ represents the likelihood for each modality. For most existing multimodality generative models, the prior distribution is assumed to be a non-informative uni-modal distribution, such as Gaussian or Laplacian. In this work, we propose to formulate the prior $p_{\alpha}(z)$ as an EBM prior \cite{pang2020learning}, which takes the form shown in Eqn. \ref{eqn:model_ebm},
\vspace{-2mm}
{
\begin{equation}
\begin{aligned}
\label{eqn:model_ebm}
&p_{\alpha}(z) = \frac{1}{Z(\alpha)}\exp [f_{\alpha}(z)] \cdot p_0(z)
% ;;;; \text{where} ;;;; p_0(z) \sim \mathcal{N}(0, I_D) \
\end{aligned}
\end{equation}
}
where $Z(\alpha)$ is a normalizing constant $Z(\alpha) = \int_z \exp [f_{\alpha}(z)] \cdot p_0(z) dz$, $p_0(z)$ is a uni-modal distribution, such as Gaussian white noise, with $p_0(z) \sim \mathcal{N}(0, I_D)$.\\
The factorized likelihood is calculated using a generator parameterized by a neural network $g_{\beta}(z) + \epsilon$. Specifically, $p_{\beta}(x|z)$ follows a predefined distribution, which is normally Gaussian or Laplacian, with $\epsilon \sim \mathcal{N}(g_{\beta}(z), I_D)$.

\noindent \textbf{Mixture of Expert (MOE)} In multimodal contexts, we adopt the mixture of experts framework \cite{shi2019variational} as $q_{\phi}(z|X) = \sum_{i=1}^m w_i q_{\phi}(z|x^{(i)})$ to aggregate latents from data across different modalities, where $q_{\phi}(z|x^{(i)}) \sim \mathcal{N}(u_{\phi}(x^{(i)}), V_{\phi}(x^{(i)}))$, and $w_i$ is a weight factor for each modality with $\sum_{i=1}^m w_i = 1$. We assume equal weight for each modality in our experiments.\\
\noindent \textbf{Connection to MOE with Modality Prior}
In the MMVAE+ framework \cite{palumbo2023mmvae+}, modality priors are utilized for cross-generation, with $p(z)$ indicating the Laplacian prior and $p(w)$ the modality prior. We substitute the Laplacian prior $p(z)$ with an EBM prior $p_{\alpha}(z)$, enhancing the original MOE model and its modality prior variants. For further details on MMVAE+, see \cite{palumbo2023mmvae+}.
% {
% {
% \small
% \begin{equation}
% \begin{aligned}
% \label{eqn:multi_inference}
% &
% \end{aligned}
% \end{equation}
% }
\subsection{Learning: MLE}
\noindent \textbf{Learning EBM} For the prior model, due to the intractability of the normalizing constant $Z(\alpha)$ in Eqn. \ref{eqn:model_ebm}, we cannot directly learn the model. Considering an identity in the MLE learning scheme, $E_{\theta}[\frac{\partial \log p_{\theta}(x)}{\partial \theta}]=0$ \cite{pang2020learning}, we can cancel the normalizing term, thus avoiding the intractability problem by taking gradients as shown in Eqn. \ref{eqn: grad_ebm}.
\vspace{-3mm}
{
\small
\begin{equation}
\begin{aligned}
\label{eqn: grad_ebm}
E_{z \sim p_{\theta}(z|x)}\left[\frac{\partial}{\partial \alpha} f_{\alpha}(z)\right] - E_{z \sim p_\alpha(z)}\left[\frac{\partial}{\partial \alpha} f_{\alpha}(z)\right]
\end{aligned}
\end{equation}
}\\
\noindent \textbf{Posterior Inference and Prior Sampling} From Eqn. \ref{eqn: grad_ebm}, we observe that learning an EBM requires two sampling steps: one from the EBM prior and the other from the posterior distribution. Due to the intractability of the true posterior, MCMC sampling from the generator's posterior, initiated with Gaussian noise, proves ineffective in multimodal settings. Therefore, we employ a separate inference model to effectively initiate Langevin dynamics (LD). The posterior from variational inference can serve as a warm-up stage to initialize informative LD.
{
\begin{equation}
\begin{aligned}
\label{eqn: ld_prior}
&z_{\tau+1} = z_{\tau} - \frac{s^2}{2}\frac{\partial}{\partial z}[\log {\pi}(z_{\tau})] + s\cdot\epsilon_{\tau}
\end{aligned}
\end{equation}
}
Where ${\pi}(z)$ represents $p_{\alpha}(z)$ in prior sampling, and $p_{\theta}(z|x)$ in posterior sampling.
Sampling from the EBM prior can be achieved by conducting MCMC sampling using LD, where $s$ is the step size, $\epsilon_{\tau}$ represents Gaussian noise $\epsilon_{\tau} \sim \mathcal{N}(0,I_d)$, and $\tau$ is the time step in LD. We utilize a Laplacian distribution as the initial distribution (i.e., $z_0 \sim \mathcal{N}(0, I_d)$) and conduct short-run Langevin dynamics \cite{nijkamp2019learning,nijkamp2020anatomy}.
Sampling from $p_{\theta}(z|x)$ can also be achieved with LD, iterating through inferential backpropagation where $s$ is the inferential step size. \\
\noindent \textbf{Connection to ELBO}
We employ MLE to jointly train the EBM prior and MCMC-based inference for the multimodal generative model. \
{
\small
\begin{equation}
\begin{aligned}
\label{eqn:mle}
L(\theta)
&= \sum_{i=1}^n \log \int_z p_{\alpha}(z)p_{\beta}(x_i^{(1)}|z)\cdots p_{\beta}(x_i^{(m)}|z)dz
\end{aligned}
\end{equation}
}
Where $\theta$ comprises learning parameters $(\alpha, \beta, \phi)$: $\alpha$ for EBM parameters, $\beta$ for generator parameters, and $\phi$ for inference model parameters. Learning the EBM, inference model, and generator jointly through MLE involves taking gradients of the objectives in Eqn. \ref{eqn:mle}. With a large number of samples $n$, maximizing Eqn. \ref{eqn:mle} is equivalent to minimizing the KL-divergence, i.e., $\text{KL}(p_{data}(X) \parallel p_{\theta}(X))$ \cite{han2019divergence}.
{
\small
\begin{equation}
\begin{aligned}
\label{eqn: mle_grad}
\frac{\partial}{\partial \theta} L(\theta) = E_{p_{\theta}(z|X)}\left[\frac{\partial}{\partial \theta} \log p_{\theta}(X,z)\right]
\end{aligned}
\end{equation}
}
Taking gradients with respect to $\alpha$ to learn the EBM yields a form similar to Eqn. \ref{eqn: grad_ebm}. Gradients with respect to $\beta$ and $\phi$ lead to Eqn. \ref{eqn: grad_generator} and Eqn. \ref{eqn: grad_inf}, closely related to the ELBO of VAEs. Given equal weights for multimodal inputs, this becomes the average of the ELBO over modalities.

\noindent \textbf{Learning Generator}
Learning the generator involves two steps: the first is inferential backpropagation from Eqn. \ref{eqn: ld_prior}, initialized from variational inference. The second step uses MCMC-inferred latents to generate data and update parameters, as shown in Eqn. \ref{eqn: grad_generator} \cite{han2017alternating}
{
\small
\begin{equation}
\begin{aligned}
\label{eqn: grad_generator}
&\frac{\partial}{\partial \beta}L(\theta,\phi)=\frac{\partial}{\partial \beta} \frac{1}{m}\sum_{i=1}^m E_{M_{\theta}^{z}q_{\phi}(z|x)} \left[\log p_{\beta_i}(x^{(i)}|z)\right]
\end{aligned}
\end{equation}
}
where $M_{\theta}^{z}$ denotes MCMC inference with LD, sampling $z$ from variational inference as a warm start.

\noindent \textbf{Learning Inference Model}
Learning the inference model can follow the ELBO, replacing $p(z)$ with the EBM prior $p_{\alpha}(z)$ and using latents from MCMC inference, denoted as $M_{\theta}^{z}$ in Eqn.\ref{eqn: grad_inf} and obtain $\frac{\partial}{\partial \phi}L(\theta,\phi)$ in the following form:
{
\footnotesize
\begin{equation}
\begin{aligned}
\label{eqn: grad_inf}
\frac{\partial}{\partial \phi} \frac{1}{m}\sum_{i=1}^m E_{M_{\theta}^{z}q_{\phi}(z|x)} \left[\log p_{\beta_i}(x^{(i)}|z) - \text{KL}(q_{\phi_i}(z|x^{(i)})\parallel p_{\alpha}(z))\right]
\end{aligned}
\end{equation}
}



% \textbf{Maximum Likelihood Learning with Variational Inference}

% \textbf{Perturbation of Maximum Likelihood}








==> sec/3_method_v2.tex <==
\section{Methodology}
\subsection{MLE}
Maximize model $p_{\theta}(X)$ equal to minimize Kullback–Leibler (KL) divergence between true data distribution $p_\text{data}(X)$ and modeled data distribution $p_{\theta}(X)$ as in Eqn.\ref{eqn:mle}. For latent generative model, complete data is denoted as $(X,z)$, so wen can further have joint distribution of latent generative model in terms of complete data as $p_\text{data}(X, z)$ and $p_{\theta}(X, z)$. 
\begin{equation}
    \begin{aligned}
        logp_{\theta}(X) &= \int_z log p_{\theta}(X,z)dz\\
    \end{aligned}
\end{equation}
\begin{equation}
    \begin{aligned}\label{eqn:mle}
    \max_{\theta} logp_{\theta}(X) &= \min_{\theta} \quad \text{KL} \left[p_{\text{data}}(X) \parallel p_{\theta}(X) \right], \\
    &= \min_{\theta} \quad \text{KL}\left[p_\text{data}(X, z) \parallel p_{\theta}(X, z)\right]
    \end{aligned}
\end{equation}
KL divergence between true distribution $p_\text{data}(X, z)$ and $p_{\theta}(X, z)$ can also be written as form in Eqn. \ref{eqn:kl}
\begin{equation}
    \begin{aligned}\label{eqn:kl}
        &\text{KL}\left[p_{\text{data}}(X, z) \parallel p_{\theta}(X, z)\right]\\
&=\int_{p_\text{data}(X,z)}p_\text{data}(X,z)log\frac{p_\text{data}(X,z)}{P_{\theta}(X,z)} dXdz \\
&=E_{p_{\text{data}}(X,z)}  \left [\log \frac{p_{\text{data}}(X,z)}{p_{\theta}(X,z)}\right]
    \end{aligned}
\end{equation}
We can further factorize joint distribution of complete data $(X,z)$ into marginal distribution as in Eqn. \ref{eqn:joint_fact}. 
\begin{equation}
    \begin{aligned}\label{eqn:joint_fact}
        &p_{\text{data}}(X,z) = p_{\text{data}}(X) q_{\phi}(z|X), \\
        &p_{\theta}(X, z) = p_{\theta}(X) p_{\theta}(z|X), \\  
    \end{aligned}
\end{equation}
And we have the MLE with expectation of $p_{\theta}(z|X)$ as in Eqn.\ref{eqn:mle_ptheta} and  the factorized KL divergence between $p_\text{data}(X, z)$ and $p_{\theta}(X, z)$ as in Eqn. \ref{eqn:kl_fact}
\begin{equation}
    \begin{aligned}\label{eqn:mle_ptheta}
        logp_{\theta}(X) =E_{p_{\theta}(z|X)} logp_{\theta}(X,z)
    \end{aligned}
\end{equation}
\begin{equation}
    \begin{aligned}\label{eqn:kl_fact}
        &\text{KL}\left[p_{\text{data}}(X, z) \parallel p_{\theta}(X, z)\right] \\
        &= \text{KL}\left[ p_\text{data}(X)q_{\phi}(z|X)\parallel p_{\theta}(X)p_{\theta}(z|X)\right]\\
        &= \text{KL} \left[p_\text{data}(X) \parallel p_{\theta}(X) \right] + \text{KL} \left[ q_{\phi} (z|X) \parallel p_{\theta}(z|X) \right]
    \end{aligned}
\end{equation}
Our goal is to minimize the KL divergence between $p_\text{data}(X, z)$ and $p_{\theta}(X, z)$ which equal to minimize the first KL divergence between true data density $p_\text{data}(X)$ and modeled data density $p_{\theta}(X)$, and second KL between generator posterior $q_{\phi}(z|X)$ and true posterior $p_{\theta}(z|X)$. True data distribution is provided and fixed, we can minimize the first KL by learning $p_{\theta}(X)$ through MLE Eqn. \ref{eqn:grad_mle}. Since $p_{\theta}(z|X)$ is intractable, we can re-write MLE with expectation of $q_{\phi}(z|X)$ as the approximate format in Eqn. \ref{eqn:grad_mle}.
\begin{equation}
    \begin{aligned}\label{eqn:grad_mle}
        \frac{\partial}{\partial \theta} L({\theta}) &=E_{p_{\theta}(z|X)}\frac{\partial}{\partial \theta}logp_{\theta}(X,z) \\
        &\sim E_{q_{\phi}(z|X)}\frac{\partial}{\partial \theta}logp_{\theta}(X) q_{\phi}(z|X)
    \end{aligned}
\end{equation}
Joint distribution $p_{\theta}(X,z)$ can also be factorized as in Eqn. \ref{eqn:2form_fact} with prior knowledge and likelihood.
\begin{equation}
    \begin{aligned}\label{eqn:2form_fact}
        p_{\theta}(X,z) &= p_{\theta}(X) p_{\theta}(z|X)\\
        &=p_{\alpha}(z)p_{\beta}(X|z)
    \end{aligned}
\end{equation}
Combining Eqn. \ref{eqn:grad_mle} and \ref{eqn:2form_fact}, we have the following MLE  as show in Eqn .\ref{eqn:new_mle} in terms of prior and likelihood:
\begin{equation}
    \begin{aligned}\label{eqn:new_mle}
        \frac{\partial}{\partial \theta} L({\theta}) &\sim E_{q_{\phi}(z|X)}\frac{\partial}{\partial \theta} logp{\alpha}(z) p_{\beta}(X|z)
    \end{aligned}
\end{equation}
Where $\theta$ contains parameter for the prior model $\alpha$, inference model $\phi$ and generator $\beta$. In our work, we proposed to use EBM prior replace uni-model prior and use MLE to learn EBM. So we can jointly train both EBM and inference model and generator through MLE.  \\
For the second KL term, true posterior $p_{\theta}(z|X)$ is intractable and we learn a proxy posterior to approximate the true form. We have three ways to obtain the proxy posterior $q_{\phi}(z|X)$. First is through generator posterior, which is initialized finite steps MCMC from Gaussian (denoted as $M_{\phi}^{z}p_0(z)$).  Second is by adding additional inference model to obtain proxy posterior through variational inference. Third is taking advantage of variational inference model which can provide a closer proxy posterior than Gaussian to take fewer steps MCMC (denoted as $M_{\phi}^{z}q_{\phi}(z|X)$) and get more closer to true form. In this work, we use Langevin dynamic to make MCMC inference as in Eqn. \ref{eqn:ld}:
\begin{equation}
    \begin{aligned}\label{eqn:ld}
        &z_{\tau+1} = z_{\tau} - \frac{s^2}{2}\frac{\partial}{\partial z}[\log q_{\phi}(z|X)] + s\cdot\epsilon_{\tau}
    \end{aligned}
\end{equation}
By takeing MCMC inference with innitailization from variaional inferred posterior, we have a more closer form of true posterior. KL divergence between MCMC inferred posterior and true posterior is less than the second term in Eqn. \ref{eqn:kl_fact} as show in Eqn.  \ref{eqn:mcmc_kl},
\begin{equation}
    \begin{aligned}\label{eqn:mcmc_kl}
        &\text{KL} \left[p_{\theta}(z|X) \parallel q_{\phi}(z|x) \right] >  \text{KL} \left[p_{\theta}(z|X) \parallel M_{\phi}^{z}q_{\phi}(z|x) \right]  
    \end{aligned}
\end{equation}
So the MLE in Eqn. \ref{eqn:new_mle} can be re-written as the form in Eqn. \ref{eqn:tight_mle}. When MCMC takes sufficient steps $M_{\phi}^{z}q_{\phi}(z|x)$ will reach true posterior, the KL distance $M_{\phi}^{z}q_{\phi}(z|x)$ and true posterior distribution will be $0$, and gradient of the model at this point is global optimal. So the KL term in Eqn.\ref{eqn:tight_mle}  can be viewed as purterbation of MLE and provide a lower bound for MLE with expectation of variatioanl inferred posterior.
\begin{equation}
    \begin{aligned}\label{eqn:tight_mle}
            \frac{\partial}{\partial \theta} L(\theta)  &=E_{p_{\theta}(z|X)}\frac{\partial}{\partial \theta}logp_{\theta}(X,z) \\
            &= E_{M_{\phi}^{z}q_{\phi}(z)}\frac{\partial}{\partial \theta} log p{\alpha}(z) p_{\beta}(X|z)\\ 
            &+\text{KL}\left[M_{\phi}^{z}q_{\phi}(z) \parallel p_{\theta}(z|X) \right]\\
            &< E_{q_{\phi}(z|X)}\frac{\partial}{\partial \theta} logp{\alpha}(z) p_{\beta}(X|z) \\
    \end{aligned}
\end{equation}
\noindent \textbf{Learn EBM}
\begin{equation}
\begin{aligned}
\label{eqn:model_ebm}
&p_{\alpha}(z) = \frac{1}{Z(\alpha)}\exp [f_{\alpha}(z)] \cdot p_0(z)
% ;;;; \text{where} ;;;; p_0(z) \sim \mathcal{N}(0, I_D) \
\end{aligned}
\end{equation}
\noindent \textbf{Learn Generator}
\begin{equation}
    \begin{aligned}\label{eqn:model_gen}
    &p_{\beta}(X, z) = p_{\beta}(X|z)p(z)\\
    &\tilde{x} = g_{\beta}(X|z) + \epsilon ,  \epsilon \sim \mathcal{N}(0, I_D),\\
    &p_{\beta}(X|z) \sim \mathcal{N}(g_{\beta}(X|z) , I_D)    
    \end{aligned}
\end{equation}
\noindent \textbf{Learn Inference Model}
\begin{equation}
    \begin{aligned}\label{eqn:model_inf}
    p_{\theta}(X,z) &= p_{\theta}(X) p_{\theta}(z|X) 
    \end{aligned}
\end{equation}


% \begin{equation}
%     \begin{aligned}\label{}
        
%     \end{aligned}
% \end{equation}


% \begin{equation}
%     \begin{aligned}\label{}
        
%     \end{aligned}
% \end{equation}


% \begin{equation}
%     \begin{aligned}\label{}
        
%     \end{aligned}
% \end{equation}


% \begin{equation}
%     \begin{aligned}\label{}
        
%     \end{aligned}
% \end{equation}


==> sec/3_prelims.tex <==
\section{Preliminaries}
\noindent \textbf{Multimodal Generative Model}
Multimodal generative models aim to learn the joint distribution of multimodal data. Suppose there are $M$ modalities; data in each modality is denoted as $x^{m}$, the entire dataset is denoted as $X = (x^{1}, x^{2} \cdots x^{m})$, and the shared latent variable is denoted as $z$. The joint probability $p(z,X)$ can be factorized into Eqn. \ref{eqn:joint_fact}. 
{
\small
\begin{equation}
    \begin{aligned}\label{eqn:joint_fact}
        p(z,X) = p(z)\prod p(x^{1}|z)p(x^{2}|z) \cdots p(x^{m}|z)
    \end{aligned}
\end{equation}
}

{\noindent Most multimodal models learn $p(z,X)$ through a shared latent variable. In multimodal generative models, VAE-based models can learn such shared latents through two foundation aggregation approach: POE \cite{wu2018multimodal} and MOE \cite{shi2019variational}, with MOE being the more commonly adopted one  \cite{sutter2020multimodal,sutter2021generalized,hwang2021multi,palumbo2023mmvae+}. MOE averages latent variables from each modality, given by $q_{\Phi}(z|X) = \frac{1}{M} \sum_{m=1}^M q_{\phi m}(z|x^{m})$. Learning such models typically adopting ELBO as in traditional VAE models, as shown in Eqn.\ref{eqn:obj_moe}.}
{
\footnotesize
\begin{equation}
    \begin{aligned}\label{eqn:obj_moe}
    &L_\text{MOE}({\theta}) =  \frac{1}{M} \sum_{m=1}^{M} \left[E_{q_{\phi_{m}}(z|x^{m})} \log \frac{p_{\beta}(z, X)}{q_{\phi_{m}}(z|x^{m})} \right]\\
    % &= \frac{1}{M} \sum_{m=1}^{M} \left[E_{q_{\phi_{m}}(z|x^{m})} \log \frac{p_{\beta}(X|z) p(z)}{q_{\phi_{m}}(z|x^{m})} \right]\\
    % &= \frac{1}{M} \sum_{m=1}^{M} \left[E_{q_{\phi}(z|x^{m})} \log p_{\beta}(x^{m}|z) + E_{q_{\phi m}(z|x^{m})} \log \frac{p(z)}{q_{\phi m}(z|x^{m})} \right]\\
    &= \frac{1}{M} \sum_{m=1}^{M} \left[E_{q_{\phi_{m}}(z|x^{m})} \log p_{\beta_{m}}(x^{m}|z) \right.\\
    &\left.+ \sum_{\substack{n=1 \\ n \neq m}}^{M}E_{q_{\phi_{m}}(z|x^{m})} \log p_{\beta_{n}}(x^{n}|z) \right.\\
    &\left.- \text{KL}\left[q_{\phi_{m}}(z|x^{m}) \parallel p(z)\right] \right]\\
    &= E_{q_{\Phi}(z|X)} \log p_{\beta}(X|z) - \text{KL}\left[q_{\Phi}(z|X) \parallel p(z)\right]
    \end{aligned}
\end{equation}
}

{\noindent Where $\theta$ comprises $(\beta, \phi)$, ${\beta}$ and ${\phi}$ denote the generator and inference model parameters, respectively. One limitation is that the objective includes a uni-modal prior $p(z)$  which cannot sufficiently capture the complexity of the multimodal data space. In this work, we propose using an expressive EBM prior $p_{\alpha}(z)$ to replace the non-informative prior.} \\
\noindent \textbf{EBM on Latent Space}
Latent space EBM aims to learn a latent distribution with high probability by assigning low energy, as shown in Eqn.\ref{eqn:model_ebm}
{
\small
\begin{equation}
    \begin{aligned}\label{eqn:model_ebm}
    &p_{\alpha}(z) = \frac{1}{Z(\alpha)}\exp [f_{\alpha}(z)] \cdot p(z)
    \end{aligned}
\end{equation}
}

{\noindent Where $Z(\alpha) = \int_z \exp [f_{\alpha}(z)] \cdot p(z) dz$ is the normalization term, $p(z)$ is uni-modal distribution as EBM prior initialization and $-f_{\alpha}(z)$ is the energy function. Learning an EBM prior in the latent space has shown promising performance on generative tasks \cite{pang2020learning, han2020joint, cui2023learning, zhang2021learning}, but the application of EBM prior in multimodal generative models is under-explored. Moreover, EBM's un-normalized exponential distribution \ref{eqn:model_ebm} provides high flexibility in modeling the latent space and enhances its effectiveness in representing the complexity of multimodal data.}

